Fusing Pruned and Backdoored Models: Optimal Transport-based Data-free Backdoor Mitigation

Backdoor attacks present a serious security threat to deep neuron networks (DNNs). Although numerous effective defense techniques have been proposed in recent years, they inevitably rely on the availability of either clean or poisoned data. In contrast, data-free defense techniques have evolved slowly and still lag significantly in performance. To address this issue, different from the traditional approach of pruning followed by fine-tuning, we propose a novel data-free defense method named Optimal Transport-based Backdoor Repairing (OTBR) in this work. This method, based on our findings on neuron weight changes (NWCs) of random unlearning, uses optimal transport (OT)-based model fusion to combine the advantages of both pruned and backdoored models. Specifically, we first demonstrate our findings that the NWCs of random unlearning are positively correlated with those of poison unlearning. Based on this observation, we propose a random-unlearning NWC pruning technique to eliminate the backdoor effect and obtain a backdoor-free pruned model. Then, motivated by the OT-based model fusion, we propose the pruned-to-backdoored OT-based fusion technique, which fuses pruned and backdoored models to combine the advantages of both, resulting in a model that demonstrates high clean accuracy and a low attack success rate. To our knowledge, this is the first work to apply OT and model fusion techniques to backdoor defense. Extensive experiments show that our method successfully defends against all seven backdoor attacks across three benchmark datasets, outperforming both state-of-the-art (SOTA) data-free and data-dependent methods. The code implementation and Appendix are provided in the Supplementary Material.

==> section/7-checklist.tex <==
\clearpage

\section*{Reproducibility Checklist}

Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

\subsection*{This paper:}

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)\\
    Answer: {\color{blue} [yes]}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)\\
    Answer: {\color{blue} [yes]}
    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper (yes/no)\\
    Answer: {\color{blue} [yes]}
\end{itemize}
\subsection*{Does this paper make theoretical contributions? (yes/no)}
Answer: {\color{blue} [yes]}

\noindent{If yes, please complete the list below.}

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)\\
    Answer: {\color{blue} [yes]}
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)\\
    Answer: {\color{blue} [yes]}
    \item Proofs of all novel claims are included. (yes/partial/no)\\
    Answer: {\color{blue} [yes]}
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)\\
    Answer: {\color{blue} [yes]}
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)\\
    Answer: {\color{blue} [yes]}
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)\\
    Answer: {\color{blue} [yes]}
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)\\
    Answer: {\color{blue} [yes]}
\end{itemize}

\subsection*{Does this paper rely on one or more datasets? (yes/no)}
Answer: {\color{blue} [yes]}

\noindent{If yes, please complete the list below.}

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets. (yes/partial/no/NA) \\
    Answer: {\color{blue} [yes]}
    \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)\\
    Answer: {\color{blue} [yes]}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)\\
    Answer: {\color{blue} [yes]}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)\\
    Answer: {\color{blue} [yes]}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)\\
    Answer: {\color{blue} [yes]}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying. (yes/partial/no/NA)
    Answer: {\color{blue} [NA]}
\end{itemize}

\subsection*{Does this paper include computational experiments? (yes/no)}
Answer: {\color{blue} [yes]}

\noindent{If yes, please complete the list below.}

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (yes/partial/no)\\
    Answer: {\color{blue} [no]}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)\\
    Answer: {\color{blue} [partial]}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)\\
    Answer: {\color{blue} [yes]}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. (yes/partial/no)\\
    Answer: {\color{blue} [yes]}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)\\
    Answer: {\color{blue} [yes]}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)\\
    Answer: {\color{blue} [partial]}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)\\
    Answer: {\color{blue} [yes]}
    \item This paper states the number of algorithm runs used to compute each reported result. (yes/no)\\
    Answer: {\color{blue} [no]}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)\\
    Answer: {\color{blue} [no]}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)\\
    Answer: {\color{blue} [yes]}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)\\
    Answer: {\color{blue} [yes]}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)\\
    Answer: {\color{blue} [yes]}
\end{itemize}
